GALA: Geometry-Aware Local Adaptive Grids for Detailed 3D Generation

We propose GALA, a novel representation of 3D shapes that (i) excels at capturing and reproducing complex geometry and surface details, (ii) is computationally efficient, and (iii) lends itself to 3D generative modelling with modern, diffusion-based schemes. The key idea of GALA is to exploit both the global sparsity of surfaces within a 3D volume and their local surface properties. Sparsity is promoted by covering only the 3D object boundaries, not empty space, with an ensemble of tree root voxels. Each voxel contains an octree to further limit storage and compute to regions that contain surfaces. Adaptivity is achieved by fitting one local and geometry-aware coordinate frame in each non-empty leaf node. Adjusting the orientation of the local grid, as well as the anisotropic scales of its axes, to the local surface shape greatly increases the amount of detail that can be stored in a given amount of memory, which in turn allows for quantization without loss of quality. With our optimized C++/CUDA implementation, GALA can be fitted to an object in less than 10 seconds. Moreover, the representation can efficiently be flattened and manipulated with transformer networks. We provide a cascaded generation pipeline capable of generating 3D shapes with great geometric detail.

==> tables/compare_property_new.tex <==
\begin{figure}[ht]
    \centering
    \begin{minipage}{0.5\textwidth}
        \centering
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{@{}lccc@{}}
        \thickhline
        \addlinespace[4pt] 
        Methods & Description of representation & \makecell{Fitting \\ Time $\downarrow$} & \makecell{Generation \\ Network} \\ 
        \midrule
        S2VS~\cite{zhang20233dshape2vecset} & Autoencoded vector set  & - & Transformer \\
        MeshDiffusion~\cite{liu2023meshdiffusion} & Deformable tetrahedral grid & 20m-30m & 3D UNet \\
        Neural Wavelet~\cite{hui2022neural} & Two levels of wavelet coefficients & 1s & 3D UNet \\
        Make-A-Shape~\cite{hui2024make} & Packed wavelet coefficients & 2s & 3D UNet \\
        Mosaic-SDF~\cite{yariv2023mosaic} & Grids on boundary & 2m & Transformer \\
        \acro (ours) & Trees with adaptive grids on boundary & 10s  & Transformer \\
        \addlinespace[4pt] 
        \thickhline
        \end{tabular}%
        }
    \end{minipage}%
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/repre_2D_plot.png} % Replace with your figure path
    \end{minipage}
    \vspace{5pt}
    \caption{Comparison of different representations for 3D generation. The table on the left highlights the properties of different methods, while the figure on the right illustrates the performance or results from these approaches.}
    \label{fig:table_and_figure}
\end{figure}

